Designing Secure Ethereum Smart Contracts: A Finite State Machine Based Approach

The adoption of blockchain-based distributed computation platforms is growing fast. Some of these platforms, such as Ethereum, provide support for implementing smart contracts, which are envisioned to have novel applications in a broad range of areas, including finance and Internet-of-Things. However, a significant number of smart contracts deployed in practice suffer from security vulnerabilities, which enable malicious users to steal assets from a contract or to cause damage. Vulnerabilities present a serious issue since contracts may handle financial assets of considerable value, and contract bugs are non-fixable by design. To help developers create more secure smart contracts, we introduce FSolidM, a framework rooted in rigorous semantics for designing con- tracts as Finite State Machines (FSM). We present a tool for creating FSM on an easy-to-use graphical interface and for automatically generating Ethereum contracts. Further, we introduce a set of design patterns, which we implement as plugins that developers can easily add to their contracts to enhance security and functionality.

==> designing-secure-ethereum (1)/accessControl.tex <==
\section{Implementation of the Access Control Plugin}
\label{sec:accessContrImpl}

%\subsubsection{Implementation}

Here, we describe the implementation of the access control plugin, which is introduced in Section~\ref{sec:accessContr}.

If the access control plugin is enabled, then
\begin{align*}
\lbl{Plugins} ~{+\!\!=} ~&\code{mapping(address => bool) private isAdmin;} \\
&\code{uint private numAdmins = 1;} \\
& \\
& \code{function } name \code{() \{} \\
& \ind \code{isAdmin[msg.sender] = true;} \\
%& \ind \code{numAdmins = 1;} \\
& \code{\}} \\
& \\
& \code{modifier onlyAdmin \{} \\
& \ind \code{require(isAdmin[msg.sender]);} \\
& \ind \code{\char`_;} \\
& \code{\}} \\
& \\
& \code{function addAdmin(address admin) onlyAdmin \{} \\
& \ind \code{require(!isAdmin[admin]);} \\
& \ind \code{isAdmin[admin] = true;} \\
& \ind \code{numAdmins += 1;} \\
& \code{\}} \\
& \\
& \code{function removeAdmin(address admin) onlyAdmin \{} \\
& \ind \code{require(isAdmin[admin]);} \\
& \ind \code{require(numAdmins > 1);} \\
& \ind \code{isAdmin[admin] = false;} \\
& \ind \code{numAdmins -= 1;} \\
& \code{\}}
\end{align*}
For transitions $t$ such that $\lbl{admin} \in t^{tags}$ (i.e., transitions that are tagged ``only admin'' by the developer), 
\begin{align*}
\lbl{TransitionPlugins}(t) ~{+\!\!=} ~&\code{onlyAdmin}
\end{align*}

==> designing-secure-ethereum (1)/concl.tex <==
\section{Conclusion and Future Work}
\label{sec:concl}

Distributed computing platforms with smart-contract functionality are envisioned to have a significant technological and economic impact in the future.
However, if we are to avoid an equally significant risk of security incidents,
we must ensure that smart contracts are secure.
While previous research efforts focused on identifying vulnerabilities in existing contracts, we explored a different avenue by proposing and implementing a novel framework for creating secure smart contracts.
%
We introduced a formal, FSM based model of smart contracts.
Based on this model, we implemented a graphical editor for designing contracts as FSMs and an automatic code generator.
We also provided a set of plugins that developers can add to their contracts.
Two of these plugins, \emph{locking} and \emph{transition counter}, implement security features for preventing common vulnerabilities (i.e., reentrancy and unpredictable state).
The other two plugins, \emph{automatic timed transitions} and \emph{access control}, implement common design patterns to facilitate the development of correct contracts with complex functionality.

%\subsection{Future Work}

We plan to extend our framework in multiple directions.
%
First, we will introduce a number of plugins, implementing various security features and design patterns. 
We will provide security plugins for all the vulnerability types identified in~\cite{atzei2017survey} that can be addressed on the level of Solidity code.
\todo{Reference the events plugins as an example?}
We will also provide plugins implementing the most popular design patterns surveyed in~\cite{bartoletti2017empirical}. 

Second, we will integrate verification tools~\cite{bensalem2009d,cavada2014nuxmv} and correctness-by-design techniques~\cite{mavridou2016satellite} into our framework.
This will enable developers to easily verify the security and safety properties of their contracts.
For example, developers will be able to verify if a malicious user could lead a contract into a deadlocked state.
Recall that deadlocks present a serious issue since it may be impossible to recover the functionality or assets of a deadlocked contract.

Third, we will enable developers to model and verify multiple interacting contracts as a set of interacting FSMs.
By verifying multiple contracts together, developers will be able to identify a wider range of issues.
For example, a set of interacting contracts may get stuck in a deadlock even if the individual contracts are deadlock free.



==> designing-secure-ethereum (1)/intro.tex <==
\section{Introduction}
\label{sec:intro}

The adoption and importance of blockchain based distributed ledgers are growing fast.
For example, the market capitalization of Bitcoin, the most-popular cryptocurrency, has exceeded \$70 billion in 2017.\footnote{\url{https://coinmarketcap.com/currencies/bitcoin/}}
%For example, the market capitalization of the blockchain based cryptocurrencies Ethereum and Bitcoin have reached \$30 and \$70 billion in 2017, respectively.
While the first generation of blockchain systems were designed to provide only cryptocurrencies, later systems, such as Ethereum, can also function as distributed computing platforms~\cite{underwood2016blockchain,wood2014ethereum}.
These distributed and trustworthy  platforms enable the implementation smart contracts, which can automatically execute or enforce their contractual terms~\cite{clack2016smart}.
Beyond financial applications, blockchains are envisioned to have a wide range of applications, such as asset tracking for the Internet-of-Things~\cite{christidis2016blockchains}.
Due to their unique advantages,
blockchain based platforms and smart contracts are embraced by an increasing number of organizations and companies.
For instance, the project HyperLedger\footnote{\url{https://www.hyperledger.org/}}, which aims to develop open-source blockchain tools, is backed by major technology companies and financial firms, such as IBM, Cisco, J.P. Morgan, and Wells Fargo~\cite{vukolic2017rethinking}.

\begin{comment}
The adoption and importance of smart contracts and distributed ledgers are growing fast:
\begin{itemize}
\item  market capitalization of cryptocurrenices is growing fast (numbers, but everyone knows this...)
\item more and more companies and organizations embrace distributed ledgers and smart contracts (may act as business enablers, distributed economy, etc.)
\item other applications, such as IoT (research papers go here)
\end{itemize}
\end{comment}

At the same time, smart contracts deployed in practice are riddled with bugs and security vulnerabilities.
A recent automated analysis of 19,336 smart contracts deployed on the public Ethereum blockchain found that 8,333 contracts suffer from at least one security issue~\cite{luu2016making}.
While not all of these issues lead to security vulnerabilities, many of them enable cyber-criminals to steal digital assets, such as cryptocurrencies.
For example, the perpetrator(s) of the infamous 2016 ``The DAO'' attack exploited a combination of vulnerabilities to steal 3.6 million Ethers, which was worth around \$50 million at the time of the attack~\cite{finley2016million}.
More recently, \$31 million worth of Ether was stolen due to a critical security flaw in a digital wallet contract~\cite{qureshi2017hacker}.
Furthermore, malicious attackers might be able to cause damage even without stealing any assets, e.g., by leading a smart contract into a deadlocked state, which does not allow the rightful owners to spend or withdraw their assets.

\begin{comment}
Smart contracts deployed in practice are ridden with bugs and security vulnerabilities:
\begin{itemize}
\item famous hacks (e.g., DAO and other multi-million dollar thefts)
\cite{finley2016million}
\item surveys on vulnerability statistics (cite research papers) 
\end{itemize}
\end{comment}

Security vulnerabilities in smart contracts present a serious issue for multiple reasons.
Firstly, smart contracts deployed in practice handle financial assets of significant value.
For example, at the time of writing, the combined value held by Ethereum contracts deployed on the public blockchain is 12,205,760 Ethers, which is worth more than \$3 billion.\footnote{\url{https://etherscan.io/accounts/c}}
Secondly, smart-contract bugs cannot be patched. 
By design, once a contract is deployed, its functionality cannot be altered even by its creator.
Finally, once a faulty or malicious transaction is recorded, it cannot be removed from the blockchain (``code is law'' principle~\cite{bhargavan2016short}).
The only way to roll back a transaction is by performing a hard fork of the blockchain, which requires consensus among the stakeholders and undermines the trustworthiness of the platform~\cite{leising2017ether}.

\begin{comment}
Smart contract bugs are a serious issues because:
\begin{itemize}
\item many contracts handle (or are envisioned to handle) expensive financial assets 
\item smart contract vulnerabilities are ``unfixable'' because
\begin{itemize}
\item smart contract code cannot be updated (by design, without this limitation smart contracts would be meaningless)
\item once a malicious transaction is recorded on the ledger it cannot be removed without a hard fork (which should be avoided at all cost, see DAO hack)
``code is law'' principle~\cite{bhargavan2016short}
\end{itemize}
\end{itemize}
\end{comment}

In practice, these vulnerabilities often arise due to the semantic gap between the assumptions contract writers make about the underlying execution semantics and the actual semantics of smart contracts~\cite{luu2016making}.
Prior work focused on addressing these issues in existing contracts by providing tools for verifying correctness~\cite{bhargavan2016short} and for identifying common vulnerabilities~\cite{luu2016making}.
%
\begin{comment}
Why are smart contracts so insecure? (cite research papers and add our thoughts)
\Natassa{I think here we need to stress the fact that security problems arise due to a semantic gap between the assumptions contract writers make about the underlying execution semantics and the actual semantics of the smart contract system. We aim to make the execution semantics clear to developers by using FSMs and provide easy to use design patterns - solutions to known vulnerabilities of smart contracts.}

Previous efforts tried to
- verify correctness (e.g.,~\cite{bhargavan2016short,hirai2016formal})
- provide tools for identifying common vulnerabilities (e.g.,~\cite{luu2016making})
We need to construct correct contracts!
\Natassa{I would leave the correctness for the next paper.}
\end{comment}
%
In this paper, we explore a different avenue by proposing and implementing \emph{FSolidM}, a novel framework for creating secure smart contracts:
\begin{compactitem}
\item We introduce a formal, finite-state machine (FSM) based model for smart contracts. We designed our model primarily to support Ethereum smart contracts, but it may be applied on other platforms as well.
\item We provide an easy-to-use graphical editor that enables developers to design smart contracts as FSMs.
\item We provide a tool for translating FSMs into Solidity code.\footnote{Solidity is the most widely used high-level language for developing Ethereum contracts. Solidity code can be translated into Ethereum Virtual Machine bytecode, which can be deployed and executed on the platform.}
\item We provide a set of plugins that implement security features and design patterns, which developers can easily add to their model.
\end{compactitem}
Our tool is open-source and available online (see Section~\ref{sec:tool} for details).

The advantages of our approach, which aims to help developers create secure contracts rather than to fix existing ones, are threefold.
First, we provide a formal model with clear semantics and an easy-to-use graphical editor, thereby decreasing the semantic gap and eliminating the issues arising from it.
Second, rooting the whole process in rigorous semantics allows the connection of our framework to formal analysis tools~\cite{bensalem2009d,cavada2014nuxmv}.
% While our tool at the moment is not capable of performing verification, it can easily be extended to include such functionality.
Finally, our code generator---coupled with the plugins provided in our tool---enables developers to implement smart contracts with minimal amount of error-prone manual coding.


==> designing-secure-ethereum (1)/numerical.tex <==
\subsection{Numerical Results on Computational Cost}
\label{sec:numerical}

Plugins not only enhance security but also increase the computational cost of transitions.
Since users must pay a relatively high price for computation performed on the public Ethereum platform, the computational cost of plugins is a critical question.
Here, we measure and compare the computational cost of transitions in our blind-auction contract without and with the locking and transition counter plugins.
We focus on these security feature plugins because they introduce overhead, while the design pattern plugins introduce useful functionality.

For this experiment, we use Solidity compiler version 0.4.17 with optimizations enabled.
In all cases, we quantify computational cost of a transition as the gas cost of an Ethereum transaction that invokes the function implementing the transition.\footnote{Gas measures the cost of executing computation on the Ethereum platform.}
The cost of deploying our smart contract was 504,672 gas without any plugins, 577,514 gas with locking plugin, 562,800 gas with transition counter plugin, and 637,518 gas with both plugins.\footnote{At the time of writing, this cost of deployment was well below \$1 (if the deployment does not need to be prioritized).}

\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
    width=1.05\textwidth,
    height=0.5\textwidth,
    bar width=0.018\textwidth,
    ybar,
    ymin=0,
    ylabel={Transaction cost [gas]},
    legend pos=north east,
    symbolic x coords={{bid}, {cancelABB}, {unbid}, {close}, {reveal}, {finish}, {withdraw}},
    xtick=data,
    xticklabel style={font=\small\tt},
    ]
    \addplot coordinates { % without locking
        (bid, 58249)        
        (cancelABB, 42059)  
        (unbid, 19735)
        (close, 42162)
        (reveal, 65729)
        (finish, 27239)
        (withdraw, 20290)
    };
    \addlegendentry{without plugins};
    \addplot coordinates { % with locking
        (bid, 68917)        
        (cancelABB, 52727)
        (unbid, 30406)
        (close, 52830)
        (reveal, 76415)
        (finish, 37913)
        (withdraw, 30961)
    };
    \addlegendentry{with locking};
    \addplot coordinates { % with counter
        (bid, 63924)        
        (cancelABB, 47661)
        (unbid, 25406)
        (close, 47764)
        (reveal, 71390)
        (finish, 32891)
        (withdraw, 25961)
    };
    \addlegendentry{with counter};
    \addplot coordinates { % with both
        (bid, 74607)        
        (cancelABB, 58329)
        (unbid, 36074)
        (close, 58432)
        (reveal, 82067)
        (finish, 43559)
        (withdraw, 36629)
    };
    \addlegendentry{with both};
\end{axis}
\end{tikzpicture}
\caption{Transaction costs in gas without plugins (\textcolor{blue}{\bf blue}), with locking plugin (\textcolor{red}{\bf red}), with transition counter plugin (\textcolor{brown}{\bf brown}), and with both plugins (\textcolor{darkgray}{\bf dark gray}).}
\label{fig:transCosts}
\end{figure}

Figure~\ref{fig:transCosts} (and Table~\ref{tab:transCosts} in Appendix~\ref{sec:numericalTable}) shows the gas cost of each transition for all four combinations of the two plugins. 
We make two key observations.
First, \emph{computational overhead is almost constant} for both plugins and also for their combination.
For example, the computational overhead introduced by locking varies between 10,668 and 10,686 gas.
For the simplest transition, \texttt{unbid}, this constitutes a 54\%  increase in computational cost,
while for the most complex transition, \texttt{reveal}, the increase is 16\%.
Second, the \emph{computational overhead of the two plugins is additive}. The increase in computational cost for enabling locking, transition counter, and both are around 10,672 gas, 5,648 gas, and 16,319 gas, respectively.





==> designing-secure-ethereum (1)/numericalTable.tex <==
\section{Numerical Results on Computational Cost -- Table}
\label{sec:numericalTable}

Table~\ref{tab:transCosts} shows the gas cost of each transition for all four combinations of the \emph{locking} and \emph{transition counter} plugins.
Please see Section~\ref{sec:numerical} for a discussion of these results.

\begin{table}
\centering
\caption{Computational Cost of Transitions}
\label{tab:transCosts}
\setlength{\tabcolsep}{0.6em}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{|l|r|r|r|r|}
\hline
Transition & \multicolumn{4}{c|}{Computational cost [gas]} \\
\cline{2-5}
 & without plugins & with locking & with transition counter & with both \\
\hline
\texttt{bid} & 58,249 & 68,917 & 63,924 & 74,607 \\
\texttt{cancelABB} & 42,059 & 52,727 & 47,661 & 58,329 \\
\texttt{unbid} & 19,735 & 30,406 & 25,406 & 36,074 \\
\texttt{close} & 42,162 & 52,830 & 47,764 & 58,432 \\
\texttt{reveal} & 65,729 & 76,415 & 71,390 & 82,067 \\
\texttt{finish} & 27,239 & 37,913 & 32,891 & 43,559 \\
\texttt{withdraw} & 20,290 & 30,961 & 25,961 & 36,629 \\
\hline
\end{tabular}
\end{table}
 

==> designing-secure-ethereum (1)/plugins.tex <==
\section{Security Extensions and Patterns}
\label{sec:plugins}

Building on the FSM model and the FSM-to-Solidity transformation introduced in the previous sections, we next provide extensions and patterns for enhancing the security and functionality of contracts.
These extensions and patterns are implemented as plugins, which are appended to the $\lbl{Plugins}$ and $\lbl{TransitionPlugins}$ elements.
Developers can easily add plugins to a contract (or some of its transitions) using our tool, without writing code manually.\footnote{Please note that we introduce an additional plugin in Appendix~\ref{sec:events}, which we omitted from the main text due to lack of space.}

\subsection{Locking}
\label{sec:locking}

To prevent reentrancy vulnerabilities, we provide a security plugin for locking the smart contract.
\footnote{\url{http://solidity.readthedocs.io/en/develop/contracts.html?highlight=mutex\#function-modifiers}}
The locking feature eliminates reentrancy vulnerabilities in a ``foolproof'' manner:  
functions within the contract cannot be nested within each other in any way.

\subsubsection{Implementation}
If the locking plugin is enabled, then
\begin{align*}
\lbl{Plugins} ~{+\!\!=} ~&\code{bool private locked = false;} \\
&\code{modifier locking \{} \\
& \ind \code{require(!locked);} \\
& \ind \code{locked = true;} \\
& \ind \code{\char`_;} \\
& \ind \code{locked = false;} \\
&\code{\}}
\end{align*}
and for every transition $t$,
\begin{align*}
\lbl{TransitionPlugins}(t) ~{+\!\!=} ~&\code{locking}
\end{align*}
Before a transition is executed, the $\texttt{locking}$ modifier first checks if the contract is locked.
If it is not locked, then the modifier locks it, executes the transition, and unlocks it after the transition has finished.
Note that the $\texttt{locking}$ plugin must be applied before the other plugins so that it can prevent reentrancy vulnerabilities in the other plugins. Our tool always applies plugins in the correct order. 

\subsection{Transition Counter}
\label{sec:transCounter}

Recall from Section~\ref{sec:commonVuln} that the state and the values of the variables stored in an Ethereum contract may be unpredictable: when a user invokes a function (i.e., transition in an FSM), she cannot be sure that the contract does not change in some way before the function is actually executed.
This issue has been referred to as ``transaction-ordering dependence''~\cite{luu2016making} and ``unpredictable state''~\cite{atzei2017survey}, and it can lead to various security issues.
Furthermore, it is rather difficult to prevent since multiple users may invoke functions at the same time, and these function invocations might be executed in any order.

We provide a plugin that can prevent unpredictable-state vulnerabilities by enforcing a strict ordering on function executions.
The plugin expects a transition number in every function as a parameter (i.e., as a transition input variable) and ensures that the number is incremented by one for each function execution.
As a result, when a user invokes a function with the next transition number in sequence, she can be sure that the function is executed before any other state changes can take place (or that the function is not executed).

\subsubsection{Implementation}
If the transition counter plugin is enabled, then
\begin{align*}
\lbl{Plugins} ~{+\!\!=} ~&\code{uint private transitionCounter = 0;} \\
&\code{modifier transitionCounting(uint nextTransitionNumber) \{} \\
& \ind \code{require(nextTransitionNumber == transitionCounter);} \\
& \ind \code{transitionCounter += 1;} \\
& \ind \code{\char`_;} \\
&\code{\}}
\end{align*}
and for every transition $t$,
\begin{align*}
\lbl{TransitionPlugins}(t) ~{+\!\!=} ~&\code{transitionCounting(nextTransitionNumber)}
\end{align*}
\todo{Clarify!}
Note that due to the inclusion of the above modifier, $t^{input}$---and hence the parameter list of every function implementing a transition--- includes the parameter $\texttt{nextTransitionNumber}$ of type $\texttt{uint}$.

\subsection{Automatic Timed Transitions}
\label{sec:timedTrans}

Next, we provide a plugin for implementing time-constraint patterns.
We first need to extend our FSM model: a Smart Contract with Timed Transitions is a tuple $C = (S, s_0, C, I, O, \rightarrow, \overset{T}{\rightarrow})$, where $\overset{T}{\rightarrow} \subseteq S \times \mathcal{G}_T \times \mathbb{N} \times \mathcal{F}_T \times S$ is a timed transition relation such that
\begin{compactitem}
\item $\mathcal{G}_T = \mathbb{B}[C]$ is a set of guards (without any input data),
\item $\mathbb{N}$ is the set of natural numbers, which is used to specify the time of the transition in seconds,
\item $\mathcal{F}_T$ is a set of action sets, i.e., a set of all ordered powerset of ${\mathbb{E}[C]}$.%\Aron{Is this still correct?}
\end{compactitem}
Notice that timed transitions are similar to non-timed transitions, but 1)~their guards and assignments do not use input or output data and 2)~they include a number specifying the transition time.

We implement timed transitions as a modifier that is applied to every function.
When a transition is invoked, the modifier checks whether any timed transitions must be executed before the invoked transition is executed. If so, the modifier executes the timed transitions before the invoked transition.

Writing such modifiers for automatic timed transitions manually may lead to vulnerabilities.
For example, a developer might forget to add a modifier to a function, which enables malicious users to invoke functions without the contract progressing to the correct state (e.g., place bids in an auction even though the auction should have already been closed due to a time limit).

\subsubsection{Implementation}
For every timed transition $tt \in \overset{T}{\rightarrow}$, the developer specifies a time $tt^{time} \in \mathbb{N}$ at which the transition will automatically happen (given that the guard condition is met).
This time is measured in the number of seconds elapsed since the creation (i.e., instantiation) of the contract.
We let $tt_1, tt_2, \ldots$ denote the list of timed transitions in ascending order based on their specified times. When the plugin is enabled,
\begin{align*}
\lbl{Plugins} ~{+\!\!=} ~&\code{modifier timedTransitions \{} \\
& \ind \lbl{TimedTransition}(tt_1) \\
& \ind \lbl{TimedTransition}(tt_2) \\
& \ind \ldots \\
& \ind \code{\char`_;} \\
& \code{\}} 
\end{align*}
where
\begin{align*}
\lbl{TimedTransition}(t) ~{::=} ~&\code{if ((state == States.}t^{from}\code{)} \\
& \ind\ind \code{\&\& (now >= creationTime + } t^{time}\code{) } \\
& \ind\ind \code{\&\& (} \lbl{Guard}(t)\code{)) \{} \\
& \ind \lbl{Statements}(t) \\
& \ind \code{state = States.}t^{to}\code{;} \\
& \code{\}}
\end{align*}

Finally, for every non-timed transition $t \in \rightarrow$, let
\begin{align*}
\lbl{TransitionPlugins}(t) ~{+\!\!=} ~&\code{timedTransitions}
\end{align*}

\subsection{Access Control}
\label{sec:accessContr}

In many contracts, access to certain transitions (i.e., functions) needs to be controlled and restricted.
\footnote{\url{http://solidity.readthedocs.io/en/develop/common-patterns.html\#restricting-access}}
For example, any user can participate in a typical blind auction by submitting a bid, but only the creator should be able to cancel the auction. 
To facilitate the enforcement of such constraints, we provide a plugin that 1) manages a list of administrators at runtime (identified by their addresses) and 2) enables developers to forbid non-administrators from accessing certain functions.
This plugin implements management functions (\texttt{addAdmin}, \texttt{removeAdmin}) for only one privileged group, but it could easily be extended to support more fine-grained access control.

Due to space limitation, the implementation of the access control plugin is in Appendix~\ref{sec:accessContrImpl}.


==> designing-secure-ethereum (1)/prelim.tex <==
%\section{Preliminaries}
%\label{sec:prelim}

%\subsection{Ethereum and Solidity}

\subsubsection{Common Vulnerabilities}
\label{sec:commonVuln}

\begin{itemize}
\item reentrancy
\item order of transactions
(``transaction-ordering dependence''~\cite{luu2016making} and ``unpredictable state''~\cite{atzei2017survey})
\item logical flaws
\Aron{This not very specific...}
\end{itemize}
\Aron{Cite papers!}

\begin{table}
\caption{Common Smart-Contract Vulnerabilities}
\centering
\begin{tabular}{|l|l|}
\hline
Vulnerability & Mitigation \\
\hline\hline
reentrancy & locking (Section~\ref{sec:locking}) \\
unpredictable state & transition counter (Section~\ref{sec:transCounter}) \\
logical flaws & access control (Section~\ref{sec:accessContr}), timed transitions (Section~\ref{sec:timedTrans}) \\
\hline
\end{tabular}
\end{table}

\Natassa{Maybe we could add a table here with a summary of the known vulnerabilities and say which ones we address with our implementation?}

==> designing-secure-ethereum (1)/related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Common Vulnerabilities and Design Patterns}
\label{sec:commonVuln} 

Multiple studies investigate and provide taxonomies for common security vulnerabilities and design patterns in Ethereum smart contracts.
In Table~\ref{tab:common}, we list the vulnerabilities that we address and the patterns that we implement in our framework using plugins.

\begin{table} [t]
\setlength{\tabcolsep}{0.75em}
\renewcommand{\arraystretch}{1.2}
\caption{Common Smart-Contract Vulnerabilities and Design Patterns}
\label{tab:common}
\centering
\begin{tabular}{|l|l|l|}
\hline
Type & Common Name & FSolidM Plugin \\
\hline\hline
\multirow{3}{*}{Vulnerabilities} & reentrancy~\cite{luu2016making,atzei2017survey} & locking (Section~\ref{sec:locking}) \\ 
\cline{2-3}
& transaction ordering~\cite{luu2016making} & transition counter (Section~\ref{sec:transCounter}) \\
& a.k.a. unpredictable state~\cite{atzei2017survey} & \\
\hline
\multirow{2}{*}{Patterns} & time constraint~\cite{bartoletti2017empirical} & timed transitions (Section~\ref{sec:timedTrans}) \\
\cline{2-3}
& authorization~\cite{bartoletti2017empirical} & access control (Section~\ref{sec:accessContr}) \\
\hline
\end{tabular}
\end{table}

Atzei et al.\ provide a detailed taxonomy of security vulnerabilities in Ethereum smart contracts, identifying twelve distinct types~\cite{atzei2017survey}.
For nine vulnerability types, they show how an attacker could exploit the vulnerability to steal assets or to cause damage. 
Luu et al.\ discuss four of these vulnerability types in more detail, proposing various techniques for mitigating them (see Section~\ref{sec:verification})~\cite{luu2016making}.
In this paper, we focus on two types of these common vulnerabilities:
\begin{compactitem}
\item Reentrancy Vulnerability: Reentrancy is one of the most well-known vulnerabilities, which was also exploited in the infamous ``The DAO'' attack.
In Ethereum, when a contract calls a function in another contract, the caller has to wait for the call to finish. 
This allows the callee, who may be malicious, to take advantage of the intermediate state in which the caller is, e.g., by invoking a function in the caller.
\item Transaction-Ordering Dependence:
If multiple users invoke functions in the same contract, the order in which these calls are executed cannot be predicted.
Consequently, the users have uncertain knowledge of the state in which the contract will be when their individual calls are executed. 
\end{compactitem}

%Focusing on the development of smart contracts,
Bartoletti and Pompianu 
identify nine common design patterns in Ethereum smart contracts, %, such as authorization and time constraints, 
and measure how many contracts use these patterns in practice~\cite{bartoletti2017empirical}.
Their results show that the two most common patterns are \emph{authorization} and \emph{time constraint}, which are used in 61\% and 33\% of all contracts, respectively. 
The also provide a taxonomy of Bitcoin and Ethereum contracts, dividing them into five categories based on their application domain.
Based on their categorization, they find that the most common Ethereum contracts deployed in practice are financial, notary, and games. 

% OLD VERSION
\begin{comment}
\subsection{Common Vulnerabilities and Design Patterns}
\label{sec:commonVuln} 

Multiple studies investigate and classify common security vulnerabilities in smart contracts.
% Making Smart Contracts Smarter
Luu et al.\ identify four classes of typical vulnerabilities in Ethereum smart contracts~\cite{luu2016making}.
\begin{compactitem}
\item Reentrancy Vulnerability: Reentrancy is one of the most well-known vulnerabilities, which was also exploited in the infamous ``The DAO'' attack.
In Ethereum, when a contract calls a function in another contract, the caller has to wait for the call to finish. 
This allows the callee, who may be malicious, to take advantage of the intermediate state in which the caller is, e.g., by invoking a function in the caller.
\item Transaction-Ordering Dependence:
If multiple users invoke functions in the same contract, the order in which these calls are executed cannot predicted.
Consequently, the users have uncertain knowledge of the state in which the contract will be when their individual calls are executed. 
\item Timestamp Dependence:
In Ethereum, a malicious participant may be able to alter the clock used in the execution of smart contracts by up to 900 seconds.\footnote{A miner can choose the timestamp of a new block maliciously; however, other miners will accept the block only if its timestamp is within a certain range of their clocks.}
As result, contracts whose correctness depends on the accuracy of the clock may be vulnerable.
\item Mishandled Exceptions:
Depending on how a function is called, an exception in the callee may or may not be propagated to the caller.
Due to the inconsistency of the propagation policy, developers can easily forget to properly handle exceptions in callee contracts.
\end{compactitem}
% A Survey of Attacks on Ethereum Smart Contracts (SoK)
Atzei et al.\ provide a more detailed taxonomy of security vulnerabilities in Ethereum smart contracts, identifying twelve distinct classes.
For nine of these classes, they show how an attacker could exploit the vulnerability to steal assets or to cause damage~\cite{atzei2017survey}. \Natassa{For me it is not clear how security vulnerabilities and security bugs are different. If they are the same, or at least similar, then we should make the connection with the previously mentioned security bugs.}
\Aron{I think that we can use ``vulnerabilities'' and ``security bugs'' interchangeably.}

% An empirical analysis of smart contracts: platforms, applications, and design patterns
Focusing on the development of smart contracts,
Bartoletti and Pompianu 
analyze Bitcoin and Ethereum contracts deployed in practice and provide a taxonomy of contracts~\cite{bartoletti2017empirical}.
They also identify nine common design patterns, such as time constraints and authorization, and quantify their usage. \Natassa{I think we need to mention how our work is related or mitigates the identified security bugs/vulnerabilities and whether we are using any of the identified design patterns (Luu et al., Atzei et al., Bartoletti et al.). Currently, Table 1 presents the correlation with two of the security bugs identified by Luu et al. but we need to do the same for the other papers. I understand that we can not actually tackle all the vulnerabilities explored with our approach. But what we can say is that this paper is a proof of concept in which we picked some of the most important identified vulnerabilities. Future work includes adding security patterns for the other vulnerabilities.}

\begin{table}
\caption{Common Smart-Contract Vulnerabilities}
\centering
\begin{tabular}{|p{2.95cm}|p{8.5cm}|}
\hline
Vulnerability & Mitigation \\
\hline\hline
reentrancy & locking (Section~\ref{sec:locking}) \\ 
\hline
transaction ordering 
(unpredictable state) & transition counter (Section~\ref{sec:transCounter}) \\
\hline
logical flaws & access control (Section~\ref{sec:accessContr}), timed transitions (Section~\ref{sec:timedTrans}) \\
\hline
\end{tabular}
\end{table}
\Natassa{where is Table 1 referenced in the text?}
\end{comment}

\subsection{Verification and Automated Vulnerability Discovery}
\label{sec:verification}

Multiple research efforts attempt to identify and fix these vulnerabilities through verification and vulnerability discovery.
% Formal Verification of Deed Contract in Ethereum Name Service
For example, Hirai first performs a formal verification of a smart contract that is used by the Ethereum Name Service~\cite{hirai2016formal}.\footnote{The Ethereum Name Service is a decentralized service, built on smart contracts, for addressing resources using human-readable names.}
However, this verification proves only one particular property and it involves relatively large amount of manual analysis.
In later work, Hirai defines the complete instruction set of the Ethereum Virtual Machine in Lem, a language that can be compiled for interactive theorem provers~\cite{hirai2017defining}.
Using this definition, certain safety properties can be proven for existing contracts.

% Short Paper: Formal Verification of Smart Contracts (2016)
Bhargavan et al.\ outline a framework for analyzing and verifying the safety and correctness of Ethereum smart contracts~\cite{bhargavan2016short}.
The framework is built on tools for translating Solidity and Ethereum Virtual Machine bytecode contracts into $F^*$, a functional programming language aimed
at program verification.
Using the~$F^*$ representations, the framework can verify the correctness of the Solidity-to-bytecode compilation as well as detect certain vulnerable patterns. % safety and functional-correctness properties of the contracts. 

% Making Smart Contracts Smarter
Luu et al.\ propose two approaches for mitigating common vulnerabilities in smart contracts~\cite{luu2016making}.
First, they recommend changes to the execution semantics of Ethereum, which eliminate vulnerabilities from the four classes that they identify in their paper.
However, these changes would need to be adopted by all Ethereum clients. 
As a solution that does not require changing Ethereum, they provide a tool called \textsc{Oyente}, which can analyze smart contracts and detect certain security vulnerabilities.

% In Code We Trust?
Fr{\"o}wis and B{\"o}hme define a heuristic indicator of control flow immutability to quantify the prevalence of contractual loopholes based on modifying the control flow of Ethereum contracts~\cite{frowis2017code}.
Based on an evaluation of all the contracts deployed on Ethereum, they find that two out of five contracts require trust in at least one third party.


%%% UNORGANIZED

\begin{comment}

% Short Paper: Formal Verification of Smart Contracts (2016)
% https://www.cs.umd.edu/~aseem/solidetherplas.pdf
Bhargavan et al.\ outline a framework for analyzing and verifying the safety and correctness of Ethereum smart contracts~\cite{bhargavan2016short}.
The framework is built on tools for translating Solidity and Ethereum Virtual Machine bytecode contracts into $F^*$, a functional programming language aimed
at program verification.
Using the~$F^*$ representations, the framework can verify the correctness of the Solidity compilation as well as certain safety and functional-correctness properties of the contracts.

% Making Smart Contracts Smarter
Luu et al.\ identify classes of typical security bugs in Ethereum smart contracts and propose two approaches for mitigating these vulnerabilities~\cite{luu2016making}.
First, they recommend changes to the execution semantics of Ethereum, which eliminate the vulnerabilities identified in the paper; however, these changes would have to be adopted by all Ethereum clients. 
As a solution that does not require changing Ethereum, they provide a tool called \textsc{Oyente}, which can analyze smart contracts and detect certain security vulnerabilities.

% A Survey of Attacks on Ethereum Smart Contracts (SoK)
Atzei et al.\ provide a taxonomy of security vulnerabilities in Ethereum smart contracts and show how attackers could exploit them to steal assets or cause damage~\cite{atzei2017survey}.

% An empirical analysis of smart contracts: platforms, applications, and design patterns
Bartoletti and Pompianu 
analyze Bitcoin and Ethereum contracts deployed in practice and provide a taxonomy of contracts~\cite{bartoletti2017empirical}.
They also identify nine common design patterns and quantify their usage.

% Formal Verification of Deed Contract in Ethereum Name Service
Hirai performs a formal verification of a smart contract that is used by the Ethereum Name Service~\cite{hirai2016formal}.
\footnote{The Ethereum Name Service is a decentralized service, built on smart contracts, for addressing resources using human-readable names.}
However, the verification proves only one particular property and it involves relatively large amount of manual analysis.

\end{comment}


==> designing-secure-ethereum (1)/rockpaperscissors.tex <==
\subsection{Rock-Paper-Scissors}

Consider a contract modeling an electronic rock-paper-scissors game.
Our finite-state machine based implementation has four {states}: 
%
\begin{enumerate}
\item \texttt{Play}, in which the two participants may submit their blinded choices (i.e., submit the hash values of their choices) if they make deposits;
\item \texttt{Reveal}, in which the participants reveal their choices; 
\item \texttt{Finished}, in which the winning participant may withdraw the deposits;
\item \texttt{Canceled}, in which the cooperating participant may withdraw the deposits (contract transitions to this state if the other participant did not submit a choice or did not reveal it in time).
\end{enumerate}

We have the following transitions:
\begin{itemize}
\item \texttt{choose} (from state \texttt{Play} to state \texttt{Play}):
submits a blinded choice and makes a deposit (tagged $\lbl{payable}$);
\item \texttt{close} (from state \texttt{Play} to state \texttt{Reveal}): starts the reveal phase if both participants submitted a blinded choice
 (timed transition, with a guard on the number of submitted choices);
\item \texttt{cancelPlay} (from state \texttt{Play} to state \texttt{Canceled}): cancels the game if one of the participants did not submit a blinded choice
 (timed transition, with a guard on the number of submitted choices);
\item \texttt{reveal} (from state \texttt{Reveal} to state \texttt{Reveal}): reveals a blinded choice;
\item \texttt{finish} (from state \texttt{Reveal} to state \texttt{Finished}): finishes the game and declares winner (timed transition, with a guard on the number of revealed choices);
\item \texttt{withdrawFinished} (from state \texttt{Finished} to state \texttt{Finished}): withdraws the deposits
 (may be called only by the winning participant);
\item \texttt{cancelReveal} (from state \texttt{Reveal} to state \texttt{Canceled}): cancels the game if one of the participants did not reveal its blinded choice
 (timed transition, with a guard on the number of revealed choices);
\item \texttt{withdrawCanceled} (from state \texttt{Canceled} to state \texttt{Canceled}): withdraws the deposits
 (may be called only by the cooperating participant).
\end{itemize}

==> designing-secure-ethereum (1)/voting.tex <==
\subsection{Voting}

Consider a voting contract, in which an administrator can assign voting rights to participants (identified using their Ethereum addresses), who may cast one vote each. 
Our finite-state machine based implementation has four {states}: 
%
\begin{enumerate}
\item \texttt{Setup}, in which administrators can add or remove participants, as well as add or remove options on which the participant may vote;
\item \texttt{Casting}, in which participants may cast their votes; 
\item \texttt{Closed}, in which the option with the most votes is declared winner;
\item \texttt{Canceled}, in which no winning option is selected.
\end{enumerate}

We have the following transitions:
\begin{itemize}
\item \texttt{addParticipant}, \texttt{removeParticipant} (from state \texttt{Setup} to state \texttt{Setup}):
adds or removes a voting participant (transition tagged $\lbl{admin}$);
\item \texttt{addOption}, \texttt{removeOption} (from state \texttt{Setup} to state \texttt{Setup}):
adds or removes a voting option (transition tagged $\lbl{admin}$);
\item \texttt{open} (from state \texttt{Setup} to state \texttt{Casting}):
begins the voting process (timed transition);
\item \texttt{cast} (from state \texttt{Casting} to state \texttt{Casting}):
casts a vote on an option (may be called only by a participant);
\item \texttt{close} (from state \texttt{Casting} to state \texttt{Closed}):
closes the voting process and declares a winning option (timed transition, with a guard on the number of votes casted);
\item \texttt{cancel} (from state \texttt{Casting} to state \texttt{Canceled}):
cancels the voting process (timed transition, with a guard on the number of votes casted).
\end{itemize}

==> prelim.tex <==
%\section{Preliminaries}
%\label{sec:prelim}

%\subsection{Ethereum and Solidity}

\subsubsection{Common Vulnerabilities}
\label{sec:commonVuln}

\begin{itemize}
\item reentrancy
\item order of transactions
(``transaction-ordering dependence''~\cite{luu2016making} and ``unpredictable state''~\cite{atzei2017survey})
\item logical flaws
\Aron{This not very specific...}
\end{itemize}
\Aron{Cite papers!}

\begin{table}
\caption{Common Smart-Contract Vulnerabilities}
\centering
\begin{tabular}{|l|l|}
\hline
Vulnerability & Mitigation \\
\hline\hline
reentrancy & locking (Section~\ref{sec:locking}) \\
unpredictable state & transition counter (Section~\ref{sec:transCounter}) \\
logical flaws & access control (Section~\ref{sec:accessContr}), timed transitions (Section~\ref{sec:timedTrans}) \\
\hline
\end{tabular}
\end{table}

\Natassa{Maybe we could add a table here with a summary of the known vulnerabilities and say which ones we address with our implementation?}

==> rockpaperscissors.tex <==
\subsection{Rock-Paper-Scissors}

Consider a contract modeling an electronic rock-paper-scissors game.
Our finite-state machine based implementation has four {states}: 
%
\begin{enumerate}
\item \texttt{Play}, in which the two participants may submit their blinded choices (i.e., submit the hash values of their choices) if they make deposits;
\item \texttt{Reveal}, in which the participants reveal their choices; 
\item \texttt{Finished}, in which the winning participant may withdraw the deposits;
\item \texttt{Canceled}, in which the cooperating participant may withdraw the deposits (contract transitions to this state if the other participant did not submit a choice or did not reveal it in time).
\end{enumerate}

We have the following transitions:
\begin{itemize}
\item \texttt{choose} (from state \texttt{Play} to state \texttt{Play}):
submits a blinded choice and makes a deposit (tagged $\lbl{payable}$);
\item \texttt{close} (from state \texttt{Play} to state \texttt{Reveal}): starts the reveal phase if both participants submitted a blinded choice
 (timed transition, with a guard on the number of submitted choices);
\item \texttt{cancelPlay} (from state \texttt{Play} to state \texttt{Canceled}): cancels the game if one of the participants did not submit a blinded choice
 (timed transition, with a guard on the number of submitted choices);
\item \texttt{reveal} (from state \texttt{Reveal} to state \texttt{Reveal}): reveals a blinded choice;
\item \texttt{finish} (from state \texttt{Reveal} to state \texttt{Finished}): finishes the game and declares winner (timed transition, with a guard on the number of revealed choices);
\item \texttt{withdrawFinished} (from state \texttt{Finished} to state \texttt{Finished}): withdraws the deposits
 (may be called only by the winning participant);
\item \texttt{cancelReveal} (from state \texttt{Reveal} to state \texttt{Canceled}): cancels the game if one of the participants did not reveal its blinded choice
 (timed transition, with a guard on the number of revealed choices);
\item \texttt{withdrawCanceled} (from state \texttt{Canceled} to state \texttt{Canceled}): withdraws the deposits
 (may be called only by the cooperating participant).
\end{itemize}

==> voting.tex <==
\subsection{Voting}

Consider a voting contract, in which an administrator can assign voting rights to participants (identified using their Ethereum addresses), who may cast one vote each. 
Our finite-state machine based implementation has four {states}: 
%
\begin{enumerate}
\item \texttt{Setup}, in which administrators can add or remove participants, as well as add or remove options on which the participant may vote;
\item \texttt{Casting}, in which participants may cast their votes; 
\item \texttt{Closed}, in which the option with the most votes is declared winner;
\item \texttt{Canceled}, in which no winning option is selected.
\end{enumerate}

We have the following transitions:
\begin{itemize}
\item \texttt{addParticipant}, \texttt{removeParticipant} (from state \texttt{Setup} to state \texttt{Setup}):
adds or removes a voting participant (transition tagged $\lbl{admin}$);
\item \texttt{addOption}, \texttt{removeOption} (from state \texttt{Setup} to state \texttt{Setup}):
adds or removes a voting option (transition tagged $\lbl{admin}$);
\item \texttt{open} (from state \texttt{Setup} to state \texttt{Casting}):
begins the voting process (timed transition);
\item \texttt{cast} (from state \texttt{Casting} to state \texttt{Casting}):
casts a vote on an option (may be called only by a participant);
\item \texttt{close} (from state \texttt{Casting} to state \texttt{Closed}):
closes the voting process and declares a winning option (timed transition, with a guard on the number of votes casted);
\item \texttt{cancel} (from state \texttt{Casting} to state \texttt{Canceled}):
cancels the voting process (timed transition, with a guard on the number of votes casted).
\end{itemize}
